The Coronal Temperatures of Low-Mass Main-Sequence Stars

Aims. We study the X-ray emission of low-mass main-sequence stars to derive a reliable general scaling law between coronal temperature and the level of X-ray activity. Methods. We collect ROSAT measurements of hardness ratios and X-ray luminosities for a large sample of stars to derive which stellar X-ray emission parameter is most closely correlated with coronal temperature. We calculate average coronal temperatures for a sample of 24 low-mass main-sequence stars with measured emission measure distributions (EMDs) collected from the literature. These EMDs are based on high-resolution X-ray spectra measured by XMM-Newton and Chandra. Results. We confirm that there is one universal scaling relation between coronal average temperature and surface X-ray flux, Fx, that applies to all low-mass main-sequence stars. We find that coronal temperature is related to Fx by Tcor=0.11 Fx^0.26, where Tcor is in MK and Fx is in erg/s/cm^2.

==> Journals.tex <==
\newcommand{\aj}{{AJ}}			
\newcommand{\araa}{{Ann.\ Rev.\ Astron.\ Astrophys.}}		
\newcommand{\apj}{{ApJ}}			
\newcommand{\apjl}{{ApJ Lett.}}		
\newcommand{\apjs}{{ApJS}}		
\newcommand{\apss}{{Ap\&SS}}		
\newcommand{\aap}{{A\&A.}}		
\newcommand{\aapr}{{A\&A~Rev.}}		
\newcommand{\aaps}{{A\&AS}}		
\newcommand{\an}{{AN}}			
\newcommand{\azh}{{AZh}}			
\newcommand{\baas}{{BAAS}}		
\newcommand{\BAIC}{{Bull.\ Astron.\ Inst.\ Czech.}}		
\newcommand{\jrasc}{{JRASC}}		
\newcommand{\memras}{{MmRAS}}		
\newcommand{\mnras}{{MNRAS}}		
\newcommand{\pra}{{Phys.~Rev.~A}}	
\newcommand{\prb}{{Phys.~Rev.~B}}	
\newcommand{\prc}{{Phys.~Rev.~C}}	
\newcommand{\prd}{{Phys.~Rev.~D}}	
\newcommand{\pre}{{Phys.~Rev.~E}}	
\newcommand{\prl}{{Phys.~Rev.~Lett.}}	
\newcommand{\pasp}{{PASP}}		
\newcommand{\pasj}{{PASJ}}		
\newcommand{\qjras}{{QJRAS}}		
\newcommand{\skytel}{{S\&T}}		
\newcommand{\solphys}{{Solar~Phys.}}	
\newcommand{\sovast}{{Soviet~Ast.}}	
\newcommand{\ssr}{{Space~Sci.~Rev.}}	
\newcommand{\zap}{{ZAp}}			
\newcommand{\nat}{{Nature}}		
\newcommand{\iaucirc}{{IAU~Circ.}}
\newcommand{\aplett}{{Astrophys.~Lett.}}
\newcommand{\apspr}{{Astrophys.~Space~Phys.~Res.}}
\newcommand{\bain}{{Bull.~Astron.~Inst.~Netherlands}}
\newcommand{\fcp}{{Fund.~Cosmic~Phys.}}
\newcommand{\gca}{{Geochim.~Cosmochim.~Acta}}
\newcommand{\grl}{{Geophys.~Res.~Lett.}}
\newcommand{\GAFD}{{Geophys.~Astrophys.~Fluid~Dyn.}}
\newcommand{\jcp}{{J.~Chem.~Phys.}}	
\newcommand{\jgr}{{J.~Geophys.~Res.}}	
\newcommand{\jqsrt}{{J.~Quant.~Spec.~Radiat.~Transf.}}
\newcommand{\memsai}{{Mem.~Soc.~Astron.~Italiana}}
\newcommand{\nphysa}{{Nucl.~Phys.~A}}
\newcommand{\physrep}{{Phys.~Rep.}}
\newcommand{\physscr}{{Phys.~Scr}}
\newcommand{\planss}{{Planet.~Space~Sci.}}
\newcommand{\procspie}{{Proc.~SPIE}}
\let\astap=\aap
\let\apjlett=\apjl
\let\apjsupp=\apjs
\let\applopt=\ao
